Robust Biharmonic Skinning Using Geometric Fields

Bounded bihramonic weights are a popular tool used to rig and deform characters for animation, to compute reduced-order simulations, and to define feature descriptors for geometry processing. They necessitate tetrahedralizing the volume bounded by the surface, introducing the possibility of meshing artifacts or tetrahedralization failure. We introduce a mesh-free and robust automatic skinning technique that generates weights comparable to the current state of the art, but works reliably even on open surfaces, triangle soups, and point clouds where current methods fail. We achieve this through the use of a specialized Lagrangian representation enabled by the advent of hardware ray-tracing, which circumvents the need for finite elements while optimizing the biharmonic energy and enforcing boundary conditions. The flexibility of our formulation allows us to integrate artistic control through weight painting during the optimization. We offer a thorough qualitative and quantitative evaluation of our method.

==> timingcomp.tex <==
\!\!&\!\!  \Hand{}\!\!&\!\!  \Penguin{}\!\!&\!\!  \Fish{}\!\!&\!\!  \Mushroom{}\!\!&\!\! \Scorpion{} \\
Vertices\!\!&\!\!  $16.10$k\!\!&\!\!  $4.97$k\!\!&\!\!  $58.10$k\!\!&\!\!  $67.08$\!\!&\!\! $766.22$k \\
Int. Vertices\!\!&\!\!  $7.24$k\!\!&\!\!  $23.74$k\!\!&\!\!  $28.41$k\!\!&\!\!  $32.32$k\!\!&\!\! $91.96$k \\
Tet. mesh (s)\!\!&\!\!  $0.51$\!\!&\!\!  $1.88$\!\!&\!\!  $2.36$\!\!&\!\!  $2.875$\!\!&\!\! $5915.04$ \\
\midrule
Ours (s)\!\!&\!\! $303.22$ \!\!&\!\! $311.86$ \!\!&\!\! $298.31$ \!\!&\!\! $302.22$ \!\!&\!\! $504.67$ \\
BBW (s)\!\!&\!\!  $45.86$\!\!&\!\!  $125.96$\!\!&\!\!  $89.88$\!\!&\!\!  $188.39$\!\!&\!\! OOM \\
QHW (s)\!\!&\!\!  $12.10$\!\!&\!\!  $12.77$\!\!&\!\!  $7.16$\!\!&\!\!  $15.13$\!\!&\!\! OOM \\
\bottomrule%


==> timings.tex <==
& \textsc{Fish} & \textsc{Mushroom} & \textsc{Hand} & \textsc{Penguin} & \textsc{Gear} & \textsc{Piggybank} & \textsc{Bunny} & \textsc{Shiba Inu} & \textsc{Scorpion} & \textsc{Beaver} \\
\midrule
Num. vertices & $10.79$k & $11.59$k & $7.99$k & $13.44$k & $25.38$k & $23.84$k & $20.90$k & $3.97$k & $50.00$k & $97.11$k \\
Num. faces & $21.57$k & $23.17$k & $15.98$k & $26.88$k & $50.75$k & $31.12$k & $27.06$k & $1.95$k & $99.99$k & $173.37$k \\
Uses GWN & No & No & No & No & Yes & Yes & Yes & No & Yes & Yes \\
\midrule
Training time (min) & $4.96$ & $5.05$ & $5.07$ & $5.20$ & $5.46$ & $5.57$ & $6.83$ & $6.99$ & $8.48$ & $13.12$ \\
Inference time (ms) & 68.18 & 51.10 & 57.50 & 67.58 & 101.00 & 86.39 & 91.27 & 52.17 & 149.58 & 1109.92 \\
\bottomrule
